SLA Decomposition for Network Slicing: A Deep Neural Network Approach

For a network slice that spans multiple technology and/or administrative domains, these domains must ensure that the slice's End-to-End (E2E) Service Level Agreement (SLA) is met. Thus, the E2E SLA should be decomposed to partial SLAs, assigned to each of these domains. Assuming a two level management architecture consisting of an E2E service orchestrator and local domain controllers, we consider that the former is only aware of historical data of the local controllers' responses to previous slice requests, and captures this knowledge in a risk model per domain. In this study, we propose the use of Neural Network (NN) based risk models, using such historical data, to decompose the E2E SLA. Specifically, we introduce models that incorporate monotonicity, applicable even in cases involving small datasets. An empirical study on a synthetic multidomain dataset demonstrates the efficiency of our approach.

==> Sections/GroundTruth.tex <==
\subsection{Ground Truth}
% \subsection{Data Generation}

% \label{sec:groundTruth}
% To the extent of our knowledge there is no relevant data available captured on a real multi-domain deployment. Here  we describe how we generate training and testing data. It is multi-domain extension of the data generation process described in~\cite{Vleeschauwer21_SLAdecomposition}.

% Domain $n$ ($\in \{1, \ldots, N\}$) only accepts SLA $(\tau_n, \theta_n)$ if its internal state (unknown to the orchestrator) is such that the new slice can be supported with that requested SLA. Similarly as in~\cite{Vleeschauwer21_SLAdecomposition} we assume that the internal state of domain $n$ can be described by one load parameter $\rho_n$. The new SLA will bring an additional load 
% \begin{equation}
%     \frac{\theta_n}{C_{n,max}}    
% \end{equation}
% where $C_{n,max}$ is a parameter that characterises the capacity of domain $n$ and the delay requirement can only be met if an additional headroom in load is foreseen. This required headroom depends on the nature of the traffic (see~\cite{Vleeschauwer21_SLAdecomposition}). If the traffic is Poisson, this headroom can be written as
% \begin{equation}
%      \frac{\tau_{n,ref}}{\tau_{n,ref} + \max \{ \tau_n -\tau_{n,prop}, 0\} } 
% \end{equation}
% where $\tau_{n,prop}$ is the propagation delay and $\tau_{n,ref}$ is a reference delay in domain $n$. Notice that this required headroom increases as the delay constraint $\tau_n$ is tightened. 
% Hence, the probability of acceptance in domain $n$ is:
% \begin{equation}
%     \mbox{Pr}[\rho_n \leq \chi_n], 
% % \chi_n = 1 - \frac{\theta_n}{C_{n,max}} - \frac{\tau_{n,ref}}{\tau_{n,ref} + \max \{ \tau_n -\tau_{n,prop}, 0\}}
% \end{equation}
% \begin{equation}
%     \chi_n = 1 - 
%         \frac{\theta_n}{C_{n,max}} -      \frac{\tau_{n,ref}}{\tau_{n,ref} + \max \{ \tau_n -\tau_{n,prop}, 0\}}
% \end{equation}

% The orchestrator only accepts the end-to-end SLA, if and only if, all domains accept the part of the SLA that they are assigned, i.e., with probability
% \begin{equation}
%     \prod_{n=1}^N \mbox{Pr}[\rho_n \leq \chi_n]
% \end{equation}
% but in principle it could accept the en-to-end SLA with probability:
% \begin{equation}
%     \mbox{Pr}[
%         \rho_1 \leq \chi_1, \ldots,
%         \rho_n \leq \chi_n, \ldots
%         \rho_N \leq \chi_N
%     ]
% \end{equation}
% which can differ from the former if the loads in the domains are statistically dependent.  In this paper we use:
% \begin{align}
%     &\mbox{Pr}[
%         \rho_1 \leq \chi_1, \ldots,
%         \rho_n \leq \chi_n, \ldots
%         \rho_N \leq \chi_N
%     ] \\ 
%     &= 
%     (1-\lambda) \prod_{n=1}^N \frac{1 - \exp(-\alpha \chi_n)}{1 - \exp(-\alpha)}
%     + \lambda \frac{1 - \exp(-\alpha \min\{\chi_n\})}{1 - \exp(-\alpha)}
% \end{align}
% where $\alpha>0$ is a form factor and $\lambda \in [0, 1]$ is a parameter that describes the correlation between domains.

%\label{sec:groundTruth}
%To the extent of our knowledge there is no relevant data available captured on a real multi-domain deployment. In this work, we follow the ground truth model and the data generation process described in~\cite{Vleeschauwer21_SLAdecomposition} to generate data for 3 domains. %Table~\ref{tab:modelParameters} shows the parameters that we used to model the 3 domains considered in this work. In all experiments the form factor was set $\alpha=4$.
% \begin{table}[htp]
%    \caption{Model parameters}
%    \label{tab:modelParameters}
%    \centering
%    \begin{tabular}{|c|c|c|c|}
%        \hline
%        domain & $\tau_{prop}$ & $\tau_{ref}$ & $C_{max}$ \\
%        \hline
%        1 & 25ms & 1ms & 5Gbps \\
%        2 & 8ms & 0.1ms & 10Gbps \\
%        3 & 8ms & 2ms & 8Gbps \\
%        \hline
%    \end{tabular}
% \end{table}
% The data (i.e. $x_i=(\tau_i, \theta_i)$ and $y_i=1$ for acceptance and $y_i=0$ for rejection) is generated by the given ground truth model in~\cite{Vleeschauwer21_SLAdecomposition} as following:
% \begin{enumerate*}
%   \item For each data point $i$, the delay $\tau_i$ and the throughput $\theta_i$ are randomly sampled from the uniform distribution over the interval $[\tau_{prop}, \tau_{max}]$ and $[0, \theta_{max}]$ respectively.
%   \item The pair $(\tau_i, \theta_i)$ is fed to the given ground truth model to obtain the corresponding acceptance probability $p_i$.
%   \item Given $p_i$, a coin toss is employed to decide whether the SLA $(\tau_i, \theta_i)$ is accepted or rejected.% Finally, we assign $a_k=1$ in case of acceptance, otherwise $a_k=0$. Note that $a_k$ is a binary value.
% \end{enumerate*}

==> Sections/acknowledgment.tex <==
\section*{Acknowledgement}

This work has been performed in the framework of the EC H2020 project DAEMON (Grant Agreement No. 101017109). 
